MultLFG: Training-free Multi-LoRA composition using Frequency-domain Guidance

Low-Rank Adaptation (LoRA) has gained prominence as a computationally efficient method for fine-tuning generative models, enabling distinct visual concept synthesis with minimal overhead. However, current methods struggle to effectively merge multiple LoRA adapters without training, particularly in complex compositions involving diverse visual elements. We introduce MultLFG, a novel framework for training-free multi-LoRA composition that utilizes frequency-domain guidance to achieve adaptive fusion of multiple LoRAs. Unlike existing methods that uniformly aggregate concept-specific LoRAs, MultLFG employs a timestep and frequency subband adaptive fusion strategy, selectively activating relevant LoRAs based on content relevance at specific timesteps and frequency bands. This frequency-sensitive guidance not only improves spatial coherence but also provides finer control over multi-LoRA composition, leading to more accurate and consistent results. Experimental evaluations on the ComposLoRA benchmark reveal that MultLFG substantially enhances compositional fidelity and image quality across various styles and concept sets, outperforming state-of-the-art baselines in multi-concept generation tasks. Code will be released.

==> Sec/X_supple.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary
% \section{Appendix}
%\section{Introduction}

In this supplementary material, we will provide the following details. 
\begin{enumerate}
    \item Training details.
    \item Theoretical and intuitive justification.
    \item Experimental setup.
    \item Image-to-latent scaling.
    
\end{enumerate}


\section{Training details}

We provide the hyperparameters for realistic and anime style in Tab.~\ref{tab:reality_hparams} and Tab.~\ref{tab:anime_hparams}.

\begin{table}[!h]
    \centering
    \caption{Hyperparameters for realistic style}
    \scalebox{1.0}{
    \begin{tabular}{cc}
    \toprule
    Hyperparameter & Values \\
    \midrule
    No. of inference step & 100 \\
    Guidance scale & 7 \\
    Cross-attention scale & 0.8 \\
    Text-to-image diffusion model & Stable Diffusion-v1~\cite{rombach2022high} \\
    Number of DWT components & 4\\
    DWT filter & 'Haar'\\
    \bottomrule
    \end{tabular}}
    \label{tab:reality_hparams}
\end{table}

\begin{table}[!h]
    \centering
    \caption{Hyperparameters for anime style}
    \scalebox{1.0}{
    \begin{tabular}{cc}
    \toprule
    Hyperparameter & Values \\
    \midrule
    No. of inference step & 200 \\
    Guidance scale & 10 \\
    Cross-attention scale & 0.8 \\
    Text-to-image diffusion model & Stable Diffusion-v1~\cite{rombach2022high} \\
    Number of DWT components & 4\\
    DWT filter & 'Haar'\\
    \bottomrule
    \end{tabular}}
    \label{tab:anime_hparams}
\end{table}

\vspace{-0.3cm}
\section{Theoretical and intuitive justification}
\vspace{-0.3cm}

\begin{lemma}[Frequency decomposition reduces interference]
Let \( x \) represent an image composed of multiple concepts \( \{c_i\}_{i=1}^n \). Consider wavelet decomposition of the image into frequency-specific subbands \( b \in \{LL, LH, HL, HH\} \):
$x = \sum_{b \in \{LL,LH,HL,HH\}} x_b.$

Define interference between concepts \( c_i \) and \( c_j \) within a subband \( b \) as:
\[
I_b(c_i, c_j) = \frac{\langle x_b^{c_i}, x_b^{c_j} \rangle}{\|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2}.
\]
Then, interference in the frequency domain is strictly lower than the spatial domain interference:
\[
|I_b(c_i, c_j)| \leq |I_{\text{spatial}}(c_i, c_j)|,
\]
with equality only if \( x_b^{c_i} \) and \( x_b^{c_j} \) perfectly align spatially and frequency-wise.
\end{lemma}

\begin{proof}
Consider the spatial domain representations \( x^{c_i} \) and \( x^{c_j} \) for two distinct concepts \( c_i \) and \( c_j \). By the Cauchy–Schwarz inequality:
\[
|\langle x^{c_i}, x^{c_j} \rangle| \leq \|x^{c_i}\|_2 \|x^{c_j}\|_2.
\]
Equality holds only when \( x^{c_i} \) and \( x^{c_j} \) are linearly dependent. After wavelet decomposition, the spatial domain vectors are partitioned into frequency-specific vectors \( x_b^{c_i} \) and \( x_b^{c_j} \). Thus:
\[
|\langle x_b^{c_i}, x_b^{c_j} \rangle| \leq \|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2.
\]
Because wavelet decomposition distributes the original spatial features into separate subbands, reducing direct spatial overlap, it follows that:
\[
|I_b(c_i, c_j)| = \frac{|\langle x_b^{c_i}, x_b^{c_j} \rangle|}{\|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2} \leq \frac{|\langle x^{c_i}, x^{c_j} \rangle|}{\|x^{c_i}\|_2 \|x^{c_j}\|_2} = |I_{\text{spatial}}(c_i, c_j)|.
\]
Equality is only achieved when \( x_b^{c_i} \) and \( x_b^{c_j} \) precisely align in both frequency and spatial domains, which is highly unlikely in practice due to the nature of wavelet decomposition.
\end{proof}

\section{Experimental setup.}

We conduct our experiments using the ComposeLoRA testbed~\cite{zhong2024multi}, which includes two subsets of LoRAs representing realistic and anime styles. Each subset consists of 22 LoRAs spanning 3 characters, 2 clothing types, 2 styles, 2 backgrounds, and 2 objects. The evaluation involves 480 unique composition sets, categorized as 48 sets with 2 LoRAs, 144 sets with 3 LoRAs, 192 sets with 4 LoRAs, and 96 sets with 5 LoRAs. To maintain compositional consistency, each set includes one character LoRA, ensuring no category overlaps. 
Following ComposeLoRA~\cite{zhong2024multi}, we use the composeLoRA testbed for our experiments. It consists of two unique subsets of LoRAs representing realistic and anime styles. Each subset comprises a variety of elements: 3 characters, 2 types of clothing, 2 styles, 2 backgrounds, and 2 objects, culminating in a total of 22 LoRAs in ComposLoRA. Thus, the ComposLoRA evaluation incorporates a total of 480 distinct composition sets. This includes 48 sets comprising 2 LoRAs, 144 sets with 3 LoRAs, 192 sets featuring 4 LoRAs, and 96 sets containing 5 LoRAs. It was make sure that each set include one character LoRA and avoid duplication of element categories to prevent conflicts.

To evaluate the composition of concepts, we use CLIP-score~\cite{zou2025cached} as an evaluation metric, which measure the alignment between text and images. Although existing metrics can measure the alignment between text and images, they often lack the nuance needed to assess the finer details of specific elements within an image and the overall quality of their composition. Recently, multimodal large language models like GPT-4V have demonstrated strong performance across a range of multimodal tasks, highlighting their potential for evaluating image generation. In this work, we harness GPT-4V’s capabilities to serve as an evaluator for composable image generation. We adopt a comparative evaluation strategy in which GPT-4V rates generated images along two dimensions: composition quality and image quality. Each image is scored on a scale from 0 to 10, with higher scores reflecting better quality. To guide the evaluation, GPT-4V is provided with a prompt containing the key attributes of the target composition, clear scoring criteria for both dimensions, and an expected response format. Full details of the evaluation prompts and results can be found in the Appendix. This setup enables a systematic comparison of our proposed methods against the LoRA Merge, LoRA-switch, and LoRA-composite baselines.

\textbf{User study.} Since perceptual metrics are not always reliable, we also conducted a human preference study using Amazon Mechanical Turk (AMT) for assesing the compositionality and quality. We asked 50 unbiased users rank our method against
baselines, totaling 1000 questionnaires. The aggregate responses showed that MultLFG generated images significantly outperformed baselines.

\section{Image-to-latent scaling}
The detailed algorithm for image-to-latent scaling is provided in Alg.~\ref{alg:img2latent}.

\begin{algorithm}[!t]
\caption{Img2Latent : Image Delta to Latent Delta Transform}\label{alg:img2latent}
\begin{algorithmic}

\State \textbf{Input:} Image $x\in\mathbb{R}^{H\times W\times C}$, Wavelet-domain perturbation $\Delta \hat{x} = \left( \Delta x_{LL}, \Delta x_{HL}, \Delta x_{LH}, \Delta x_{HH} \right)$, Encoder $E(\cdot)$ (e.g., VAE encoder), Inverse wavelet transform $\text{IDWT}$, Perturbation magnitude $\epsilon > 0$

\State \textbf{Output:} Latent-space delta $\Delta z$ and, optionally, its decomposition $\left( \Delta z_{LL}, \Delta z_{HL}, \Delta z_{LH}, \Delta z_{HH} \right)$
\medskip

\State \textbf{1. Reconstruct the Image-Space Perturbation:}
\State Compute $\Delta x \gets \text{IDWT}(\Delta \hat{x})$, where
\[
\Delta \hat{x} = (\Delta x_{LL}, \Delta x_{HL}, \Delta x_{LH}, \Delta x_{HH})
\]
\medskip
\State \textbf{2. Compute the Baseline and Perturbed Latent Codes:}
\State Compute baseline latent code: $z \gets E(x)$.
\State Compute perturbed latent code: $z' \gets E(x + \Delta x_{\mathcal{F}})$.

\medskip
\State \textbf{3. Compute the Latent Delta via Finite Difference:}
\State Compute the latent difference:
\[
\Delta z \gets \frac{z' - z}{\epsilon}
\]
\medskip
\State \textbf{4. Decompose $\Delta z$ into Latent Subbands:}

\hspace{0.4cm} \For{latent subbands $i\in\{\text{LL}, \text{HL}, \text{LH}, \text{HH}\}$}{
    \State Apply projection: $\Delta z_i \gets P_i(\Delta z)$.}
\EndFor
\medskip
\State \textbf{5. Importance of Concepts in Latent space:} \[\bar{w}_{\mathcal{F}} = \sum_{\mathcal{F'} \in \{\mathrm{LL}, \mathrm{HL}, \mathrm{LH}, \mathrm{HH}\}} w_{\mathcal{F'}} * \Delta z_\mathcal{F} \]

\State \Return $\bar{w}$ 
\end{algorithmic}
\end{algorithm}








==> Sec/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It's the gist. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It will help the community. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code is provided. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Help community if accepted. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> Sec/intuition.tex <==
\section{Intuitive jutification}
Concept interference in multi-concept image generation arises when features from different concepts overlap or conflict, leading to visual artifacts such as misplaced elements or unintended blending (Fig.~\ref{fig:teaser}). This issue is particularly pronounced in spatial domain approaches, where overlapping features can result in entangled representations (e.g., LoRA-composite, switch~\cite{zhong2024multi}).

Frequency domain guidance offers a solution by decomposing images into distinct frequency components (Fig.~\ref{fig:main_arch}), allowing for more precise control over individual features. By assigning adaptive weights to different frequency bands, models can emphasize or suppress specific features, reducing the likelihood of interference. For instance, low-frequency components can capture general shapes and backgrounds, while high-frequency components can represent fine details like textures or edges~\cite{mallat1989theory}. By manipulating these components separately, it's possible to maintain the integrity of each concept within the composite image.

Previous studies have shown that operating in the frequency domain allows for better preservation of image details and reduces artifacts associated with concept blending. For example, the Wavelet-Domain Image Generation (WDIG)~\cite{zhu2023wdig} framework utilizes wavelet transforms to separate and process image components, leading to improved image quality and reduced interference. Similarly, frequency-aware guidance in diffusion models~\cite{xiao2024frequency} has been demonstrated to enhance image restoration tasks by enforcing content consistency in both spatial and frequency domains.

==> Sec/theoretical_justification.tex <==
\section{Theoretical jutification}
    

% \begin{lemma}{Linearity of Frequency Transforms:}
% Let $\mathcal{F}$ be a linear, invertible frequency transform (e.g., the Fourier or a discrete wavelet transform) that satisfies perfect reconstruction. Then for any two signals $x$ and $y$, we have:
% \[
% \mathcal{F}(x+y)=\mathcal{F}(x)+\mathcal{F}(y)
% \]
% and consequently,
% \[
% \mathcal{F}^{-1}\Bigl(\mathcal{F}(x)+\mathcal{F}(y)\Bigr)=x+y.
% \]
% \end{lemma}

% \begin{theorem}{Improved Compositionality via Frequency-Domain Guidance:}
% Let $p(x)$ be the probability density over the latent (or image) space, and define the score function as
% \[
% s(x)=\nabla_{x}\log p(x).
% \]
% Note that $s(x)$ is a highly nonlinear function of $x$. Suppose that an image (or latent) $x$ is composed of several components corresponding to different concepts:
% \[
% x=x_{1}+x_{2}+\cdots+x_{k}.
% \]
% Assume that these components are designed (or assumed) to predominantly influence different frequency bands. Let $P_l$ be a projection operator onto frequency band $l$, so that
% \[
% x=\sum_{l} P_l(x),
% \]
% with the projections $P_l(x)$ being (approximately) orthogonal:
% \[
% \langle P_l(x),P_{l'}(x)\rangle=0\quad \text{for } l\neq l'.
% \]
% Then by the linearity of $\mathcal{F}$ (Lemma 1), we have
% \[
% \mathcal{F}(x)=\sum_{l}\mathcal{F}\bigl(P_l(x)\bigr).
% \]
% Thus, if we define the frequency representation of the score function over the $l$-th band as
% \[
% S_l(x)=\mathcal{F}\bigl(P_l(x)\bigr),
% \]
% then for any two contributions (e.g., from different concepts) $s_1(x)$ and $s_2(x)$, it holds that
% \[
% \mathcal{F}\Bigl(s_1(x)+s_2(x)\Bigr)=\mathcal{F}\bigl(s_1(x)\bigr)+\mathcal{F}\bigl(s_2(x)\bigr).
% \]

% However, since the score function itself is defined as
% \[
% s(x)=\nabla_x\log p(x),
% \]
% its nonlinearity implies that in the latent domain we generally do not have:
% \[
% s(x+y)=s(x)+s(y).
% \]

% Moreover, by Parseval's theorem, the total energy (squared $L^2$ norm) of the score is preserved in the frequency domain:
% \[
% \| s(x)\|_{2}^{2}=\| \mathcal{F}(s(x))\|_{2}^{2}.
% \]
% If the contributions from different concepts predominantly occupy disjoint (or nearly disjoint) frequency bands, then the energy from each concept does not interfere with that of another. Specifically, if for two concepts $i$ and $j$ the frequency supports are disjoint, we have approximately:
% \[
% \|\mathcal{F}(s_i(x))+\mathcal{F}(s_j(x))\|_{2}^{2}\approx \|\mathcal{F}(s_i(x))\|_{2}^{2}+\|\mathcal{F}(s_j(x))\|_{2}^{2}.
% \]

% \begin{theorem}{Controlled Combination in the Frequency Domain:}  
% Assume we apply subband-specific guidance in each frequency band as
% \[
% \hat{S}_l = S_l(\text{uncond}) + s_l\Bigl[S_l(\text{cond})-S_l(\text{uncond})\Bigr],
% \]
% where $s_l$ is a guidance scale for band $l$. Then, the overall updated frequency representation is given by
% \[
% \hat{S} = \sum_{l}\hat{S}_l,
% \]
% and the inverse transform yields the updated latent representation:
% \[
% \hat{x} = \mathcal{F}^{-1}(\hat{S}) = x + \sum_{l} s_l\,\mathcal{F}^{-1}\Bigl(S_l(\text{cond})-S_l(\text{uncond})\Bigr).
% \]
% \end{theorem}

% \textit{Proof.} 
% By Lemma 1, since $\mathcal{F}$ is linear,
% \[
% \mathcal{F}(x)=\sum_l \mathcal{F}\bigl(P_l(x)\bigr).
% \]
% The score function is nonlinear in $x$, so generally,
% \[
% s(x+y)\neq s(x)+s(y).
% \] 
% However, by applying the linear frequency transform to the (possibly nonlinear) score updates, we obtain an additive structure in the frequency domain:
% \[
% \mathcal{F}\bigl(s(x)\bigr)=\sum_l S_l(x),
% \]
% and a conditional update can be written per subband:
% \[
% \hat{S}_l = S_l(\text{uncond})+s_l\Bigl[S_l(\text{cond})-S_l(\text{uncond})\Bigr].
% \]
% Parseval's theorem guarantees that the energy in the latent domain is preserved in the frequency domain:
% \[
% \| s(x)\|_{2}^{2}=\| \mathcal{F}(s(x))\|_{2}^{2}.
% \]
% Thus, if different concepts contribute to different frequency bands, their energies add without interfering, i.e.,
% \[
% \|\mathcal{F}(s_i(x))+\mathcal{F}(s_j(x))\|_{2}^{2}\approx \|\mathcal{F}(s_i(x))\|_{2}^{2}+\|\mathcal{F}(s_j(x))\|_{2}^{2}.
% \] 
% The independent treatment of each frequency band allows us to use tailored guidance scales $s_l$, resulting in an updated latent:
% \[
% \hat{x} = x + \sum_{l} s_l\,\mathcal{F}^{-1}\Bigl(S_l(\text{cond})-S_l(\text{uncond})\Bigr),
% \]
% which better preserves the individual contributions of the separate concepts compared to a single, unified pixel-domain update.

% \begin{theorem}{Variance Decomposition in Frequency-Domain Guidance:}
% Assume the frequency bands $\{P_{l}(x)\}$ are orthogonal and the contributions from different concepts are localized to different bands. Then the energy (squared $L^{2}$ norm) of the overall guidance update satisfies
% \[
% \left\|\hat{S} - \mathcal{F}(x)\right\|_{2}^{2} \approx \sum_{l}\left\| s_{l}\Bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\Bigr] \right\|_{2}^{2}.
% \]
% Moreover, by Parseval's theorem, this implies that in the latent space,
% \[
% \left\| \hat{x}-x \right\|_{2}^{2} \approx \sum_{l}\left\| \mathcal{F}^{-1}\Bigl( s_{l}\bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\bigr] \Bigr) \right\|_{2}^{2}.
% \]
% Thus, the overall variance of the update is decomposed into the sum of variances from each independent frequency band, reducing cross-band interference and leading to a more stable update.
% \end{theorem}

% \textit{Proof.}
% By the linearity of $\mathcal{F}$ (Lemma 1), we have
% \[
% \hat{S} - \mathcal{F}(x)=\sum_{l}\Bigl(S_{l}(\text{uncond}) + s_{l}[S_{l}(\text{cond})-S_{l}(\text{uncond})] - S_{l}(x)\Bigr).
% \]
% Under the assumption that each $x_{i}$ is primarily present in a specific frequency band, we have
% \[
% S_{l}(x)=S_{l}(\text{uncond}),
% \]
% for bands not affected by a particular concept. Thus, the update in each band simplifies to
% \[
% s_{l}\Bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\Bigr].
% \]
% Since the frequency bands are orthogonal, the energy of the sum is the sum of the energies:
% \[
% \left\|\hat{S} - \mathcal{F}(x)\right\|_{2}^{2} \approx \sum_{l}\left\| s_{l}\Bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\Bigr] \right\|_{2}^{2}.
% \]
% Finally, applying Parseval’s theorem ensures that the energy is preserved when transforming back to the latent space:
% \[
% \left\| \hat{x}-x \right\|_{2}^{2} \approx \left\|\hat{S} - \mathcal{F}(x)\right\|_{2}^{2}.
% \]


\begin{lemma}[Linearity of Frequency Transforms]
Let $\mathcal{F}$ be a linear, invertible frequency transform (e.g., the Fourier or Discrete Wavelet Transform) satisfying perfect reconstruction. Then for any signals $x$ and $y$:
\[
\mathcal{F}(x + y) = \mathcal{F}(x) + \mathcal{F}(y), \quad \text{and} \quad \mathcal{F}^{-1}(\mathcal{F}(x)) = x.
\]
\end{lemma}

\begin{theorem}[Improved Compositionality via Frequency-Domain Guidance]
Let $x = x_1 + x_2 + \dots + x_k$ be a latent composed of $k$ concept-specific components. Assume that each $x_i$ is mostly localized in frequency band $l_i$ via orthogonal projections $\{P_l\}$, such that
\[
x = \sum_l P_l(x), \quad \text{and} \quad \langle P_l(x), P_{l'}(x) \rangle = 0 \quad \text{for } l \neq l'.
\]
Let $s(x) = \nabla_x \log p(x)$ be the score function of a diffusion model. Then, in the frequency domain:
\[
\mathcal{F}(s(x)) = \sum_l \mathcal{F}(P_l(s(x))) = \sum_l S_l(x),
\]
and a guided update with subband-specific scales $s_l$ defined as
\[
\hat{S}_l = S_l(\text{uncond}) + s_l \left[S_l(\text{cond}) - S_l(\text{uncond})\right]
\]
yields the overall update:
\[
\hat{x} = \mathcal{F}^{-1}\left(\sum_l \hat{S}_l\right) = x + \sum_l s_l \mathcal{F}^{-1}\left(S_l(\text{cond}) - S_l(\text{uncond})\right).
\]
\end{theorem}

\textit{Proof.}
From Lemma 1, $\mathcal{F}$ is linear and invertible. Therefore,
\[
\mathcal{F}(x) = \sum_l \mathcal{F}(P_l(x)).
\]
Though $s(x)$ is nonlinear, the linearity of $\mathcal{F}$ ensures
\[
\mathcal{F}(s(x)) = \sum_l \mathcal{F}(P_l(s(x))) = \sum_l S_l(x).
\]
Subband guidance is performed independently:
\[
\hat{S}_l = S_l(\text{uncond}) + s_l\left[S_l(\text{cond}) - S_l(\text{uncond})\right],
\]
so the updated latent is given by
\[
\hat{x} = \mathcal{F}^{-1}\left(\sum_l \hat{S}_l\right).
\]
% \end{proof}

\begin{theorem}[Variance Decomposition in Frequency Guidance]
Assume the projections $P_l$ are orthogonal and concept contributions are localized in distinct bands. Then:
\[
\left\| \hat{S} - \mathcal{F}(x) \right\|_2^2 \approx \sum_l \left\| s_l \left(S_l(\text{cond}) - S_l(\text{uncond})\right) \right\|_2^2,
\]
and by Parseval’s theorem,
\[
\left\| \hat{x} - x \right\|_2^2 \approx \sum_l \left\| \mathcal{F}^{-1} \left(s_l \left[S_l(\text{cond}) - S_l(\text{uncond})\right] \right) \right\|_2^2.
\]
\end{theorem}

\textit{Proof.}
From the update definition:
\[
\hat{S} - \mathcal{F}(x) = \sum_l \left(\hat{S}_l - S_l(x)\right).
\]
For inactive bands, $S_l(x) \approx S_l(\text{uncond})$, so:
\[
\hat{S}_l - S_l(x) \approx s_l \left(S_l(\text{cond}) - S_l(\text{uncond})\right).
\]
By orthogonality:
\[
\left\| \hat{S} - \mathcal{F}(x) \right\|_2^2 \approx \sum_l \left\| s_l \left(S_l(\text{cond}) - S_l(\text{uncond})\right) \right\|_2^2.
\]
Parseval's theorem implies energy conservation under $\mathcal{F}^{-1}$, thus:
\[
\left\| \hat{x} - x \right\|_2^2 \approx \left\| \hat{S} - \mathcal{F}(x) \right\|_2^2.
\]
% \end{proof}




==> Sec/theory.tex <==
\begin{lemma}{Linearity of Frequency Transforms:}
Let $\mathcal{F}$ be a linear, invertible frequency transform (e.g., the Fourier or a discrete wavelet transform) that satisfies perfect reconstruction. Then for any two signals $x$ and $y$, we have:
\[
\mathcal{F}(x+y)=\mathcal{F}(x)+\mathcal{F}(y)
\]
and consequently,
\[
\mathcal{F}^{-1}\Bigl(\mathcal{F}(x)+\mathcal{F}(y)\Bigr)=x+y.
\]
\end{lemma}

\begin{theorem}{Improved Compositionality via Frequency-Domain Guidance:}
Let $p(x)$ be the probability density over the latent (or image) space, and define the score function as
\[
s(x)=\nabla_{x}\log p(x).
\]
Note that $s(x)$ is a highly nonlinear function of $x$. Suppose that an image (or latent) $x$ is composed of several components corresponding to different concepts:
\[
x=x_{1}+x_{2}+\cdots+x_{k}.
\]
Assume that these components are designed (or assumed) to predominantly influence different frequency bands. Let $P_l$ be a projection operator onto frequency band $l$, so that
\[
x=\sum_{l} P_l(x),
\]
with the projections $P_l(x)$ being (approximately) orthogonal:
\[
\langle P_l(x),P_{l'}(x)\rangle=0\quad \text{for } l\neq l'.
\]
Then by the linearity of $\mathcal{F}$ (Lemma 1), we have
\[
\mathcal{F}(x)=\sum_{l}\mathcal{F}\bigl(P_l(x)\bigr).
\]
Thus, if we define the frequency representation of the score function over the $l$-th band as
\[
S_l(x)=\mathcal{F}\bigl(P_l(x)\bigr),
\]
then for any two contributions (e.g., from different concepts) $s_1(x)$ and $s_2(x)$, it holds that
\[
\mathcal{F}\Bigl(s_1(x)+s_2(x)\Bigr)=\mathcal{F}\bigl(s_1(x)\bigr)+\mathcal{F}\bigl(s_2(x)\bigr).
\]

However, since the score function itself is defined as
\[
s(x)=\nabla_x\log p(x),
\]
its nonlinearity implies that in the latent domain we generally do not have:
\[
s(x+y)=s(x)+s(y).
\]

Moreover, by Parseval's theorem, the total energy (squared $L^2$ norm) of the score is preserved in the frequency domain:
\[
\| s(x)\|_{2}^{2}=\| \mathcal{F}(s(x))\|_{2}^{2}.
\]
If the contributions from different concepts predominantly occupy disjoint (or nearly disjoint) frequency bands, then the energy from each concept does not interfere with that of another. Specifically, if for two concepts $i$ and $j$ the frequency supports are disjoint, we have approximately:
\[
\|\mathcal{F}(s_i(x))+\mathcal{F}(s_j(x))\|_{2}^{2}\approx \|\mathcal{F}(s_i(x))\|_{2}^{2}+\|\mathcal{F}(s_j(x))\|_{2}^{2}.
\]

\begin{theorem}{Controlled Combination in the Frequency Domain:}  
Assume we apply subband-specific guidance in each frequency band as
\[
\hat{S}_l = S_l(\text{uncond}) + s_l\Bigl[S_l(\text{cond})-S_l(\text{uncond})\Bigr],
\]
where $s_l$ is a guidance scale for band $l$. Then, the overall updated frequency representation is given by
\[
\hat{S} = \sum_{l}\hat{S}_l,
\]
and the inverse transform yields the updated latent representation:
\[
\hat{x} = \mathcal{F}^{-1}(\hat{S}) = x + \sum_{l} s_l\,\mathcal{F}^{-1}\Bigl(S_l(\text{cond})-S_l(\text{uncond})\Bigr).
\]
\end{theorem}

\textit{Proof.} 
By Lemma 1, since $\mathcal{F}$ is linear,
\[
\mathcal{F}(x)=\sum_l \mathcal{F}\bigl(P_l(x)\bigr).
\]
The score function is nonlinear in $x$, so generally,
\[
s(x+y)\neq s(x)+s(y).
\] 
However, by applying the linear frequency transform to the (possibly nonlinear) score updates, we obtain an additive structure in the frequency domain:
\[
\mathcal{F}\bigl(s(x)\bigr)=\sum_l S_l(x),
\]
and a conditional update can be written per subband:
\[
\hat{S}_l = S_l(\text{uncond})+s_l\Bigl[S_l(\text{cond})-S_l(\text{uncond})\Bigr].
\]
Parseval's theorem guarantees that the energy in the latent domain is preserved in the frequency domain:
\[
\| s(x)\|_{2}^{2}=\| \mathcal{F}(s(x))\|_{2}^{2}.
\]
Thus, if different concepts contribute to different frequency bands, their energies add without interfering, i.e.,
\[
\|\mathcal{F}(s_i(x))+\mathcal{F}(s_j(x))\|_{2}^{2}\approx \|\mathcal{F}(s_i(x))\|_{2}^{2}+\|\mathcal{F}(s_j(x))\|_{2}^{2}.
\] 
The independent treatment of each frequency band allows us to use tailored guidance scales $s_l$, resulting in an updated latent:
\[
\hat{x} = x + \sum_{l} s_l\,\mathcal{F}^{-1}\Bigl(S_l(\text{cond})-S_l(\text{uncond})\Bigr),
\]
which better preserves the individual contributions of the separate concepts compared to a single, unified pixel-domain update.

\begin{theorem}{Variance Decomposition in Frequency-Domain Guidance:}
Assume the frequency bands $\{P_{l}(x)\}$ are orthogonal and the contributions from different concepts are localized to different bands. Then the energy (squared $L^{2}$ norm) of the overall guidance update satisfies
\[
\left\|\hat{S} - \mathcal{F}(x)\right\|_{2}^{2} \approx \sum_{l}\left\| s_{l}\Bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\Bigr] \right\|_{2}^{2}.
\]
Moreover, by Parseval's theorem, this implies that in the latent space,
\[
\left\| \hat{x}-x \right\|_{2}^{2} \approx \sum_{l}\left\| \mathcal{F}^{-1}\Bigl( s_{l}\bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\bigr] \Bigr) \right\|_{2}^{2}.
\]
Thus, the overall variance of the update is decomposed into the sum of variances from each independent frequency band, reducing cross-band interference and leading to a more stable update.
\end{theorem}

\textit{Proof.}
By the linearity of $\mathcal{F}$ (Lemma 1), we have
\[
\hat{S} - \mathcal{F}(x)=\sum_{l}\Bigl(S_{l}(\text{uncond}) + s_{l}[S_{l}(\text{cond})-S_{l}(\text{uncond})] - S_{l}(x)\Bigr).
\]
Under the assumption that each $x_{i}$ is primarily present in a specific frequency band, we have
\[
S_{l}(x)=S_{l}(\text{uncond}),
\]
for bands not affected by a particular concept. Thus, the update in each band simplifies to
\[
s_{l}\Bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\Bigr].
\]
Since the frequency bands are orthogonal, the energy of the sum is the sum of the energies:
\[
\left\|\hat{S} - \mathcal{F}(x)\right\|_{2}^{2} \approx \sum_{l}\left\| s_{l}\Bigl[S_{l}(\text{cond})-S_{l}(\text{uncond})\Bigr] \right\|_{2}^{2}.
\]
Finally, applying Parseval’s theorem ensures that the energy is preserved when transforming back to the latent space:
\[
\left\| \hat{x}-x \right\|_{2}^{2} \approx \left\|\hat{S} - \mathcal{F}(x)\right\|_{2}^{2}.
\]


\subsection{Why wavelets?}

Let $x\in\mathbb{R}^{n}$ be an image (or latent representation) and let $\mathcal{W}$ denote a discrete wavelet transform (DWT) with perfect reconstruction. Suppose $x$ is decomposed as
\[
x = x_{LL} + x_{LH} + x_{HL} + x_{HH},
\]
where $x_{LL}$ represents the low-frequency (approximation) component and $x_{LH}$, $x_{HL}$, $x_{HH}$ represent high-frequency (detail) components in different orientations. Define the guidance update in the wavelet domain as
\[
\hat{X}_b = X_b(\text{uncond}) + s_b\Bigl[ X_b(\text{cond}) - X_b(\text{uncond}) \Bigr],
\]
for each subband $b \in \{LL, LH, HL, HH\}$, where $s_b$ is a subband-specific guidance scale. Then, under the assumptions that:
\begin{enumerate}
    \item The DWT $\mathcal{W}$ is linear and has the perfect reconstruction property,
    \item The wavelet basis functions are localized in both space and frequency,
    \item The energy of $x$ is largely compacted into a few significant coefficients in each subband,
\end{enumerate}
the inverse wavelet transform yields an updated image
\[
\hat{x} = \mathcal{W}^{-1}\Bigl(\sum_{b} \hat{X}_b\Bigr),
\]
which preserves the independent contributions of the components (or concepts) with reduced cross-frequency interference. Consequently, the update in the wavelet domain is more stable and capable of enforcing both global structure and local detail, as compared to an update in the latent (or Fourier) domain where basis functions are globally supported.



\section{Overview}

Diffusion models typically transform an image \( x \) into a latent representation \( z \) via a forward noising process (and then a reverse denoising process). In parallel, a wavelet transform decomposes an image into coefficients across multiple frequency bands—each capturing details from coarse structures (low frequencies) to fine details (high frequencies). The key question is: how do perturbations (or changes) in the image---when analyzed in these wavelet bands---translate into changes in the latent space of a diffusion model?

While a direct, widely accepted theoretical analysis in the literature might be lacking, we can construct a theoretical analysis by combining ideas from linear perturbation analysis and the linearity of the wavelet transform with the (often locally) linear behavior of the encoder part of diffusion models.

\section{Theoretical Framework}

\subsection{Diffusion Process and Linearization}

In many diffusion models, the forward process can be written (at a given timestep \( t \)) as:
\[
x_t = \sqrt{\bar{\alpha}_t}\, x + \sqrt{1-\bar{\alpha}_t}\, \epsilon,
\]
where \( \epsilon \) is Gaussian noise and \(\bar{\alpha}_t\) is a time-dependent scaling factor. Suppose the latent representation is given by a function \( z = E(x) \) (where \( E \) might be non-linear). For small changes \( \Delta x \) in the image, a first-order Taylor expansion gives:
\[
\Delta z \approx J_E(x)\, \Delta x,
\]
with \( J_E(x) \) being the Jacobian (sensitivity matrix) of \( E \) at \( x \).

\subsection{Wavelet Decomposition}

The wavelet transform \( W \) is a linear and, in many cases, orthonormal operator. When you decompose \( x \) into its wavelet coefficients,
\[
\hat{x} = W(x),
\]
a small perturbation in the image translates as:
\[
\Delta \hat{x} = W(\Delta x).
\]
Because the wavelet transform is linear, it cleanly separates changes in \( x \) into contributions from different frequency bands.

\subsection{Relating the Two Domains}

Rewriting the image perturbation in terms of wavelet coefficients, we have:
\[
\Delta x = W^{-1}(\Delta \hat{x}).
\]
Substituting into the linearized latent change:
\[
\Delta z \approx J_E(x)\, W^{-1} (\Delta \hat{x}).
\]
Defining the composite linear operator
\[
A = J_E(x)\, W^{-1},
\]
the relation becomes:
\[
\Delta z \approx A\, \Delta \hat{x}.
\]
Here, \( A \) maps changes in the wavelet domain (i.e., specific frequency bands) to changes in the latent domain. Its structure---specifically, how its singular values or eigenvalues distribute across the frequency components---determines the sensitivity of \( z \) to perturbations in each wavelet band.

\section{Frequency-Band Specific Effects}

\subsection{Low Frequencies}
Low-frequency bands capture the overall structure of the image. Since these components tend to be robust to noise, the diffusion process (especially during the early stages of the reverse process) may exhibit a relatively stable mapping from these wavelet coefficients to the latent representation.

\subsection{High Frequencies}
High-frequency bands represent fine details and are often more susceptible to noise. In many diffusion models, the reverse process has to ``recover'' these details from noisy observations. The Jacobian \( J_E(x) \) might have larger variations (or even a ``spectral bias'') in these bands, meaning that small perturbations in high-frequency coefficients could lead to amplified changes in the latent representation---or, conversely, the model might learn to dampen these changes to ensure stability.

\subsection{Interplay via \( A = J_E(x)\, W^{-1} \)}
The mapping \( A \) encodes the net effect of the model's sensitivity (via \( J_E(x) \)) and the distribution of image content across wavelet bands (via \( W^{-1} \)). By analyzing \( A \)'s spectrum, one could theoretically determine which frequency bands are more influential in the latent space. For example, if \( A \) has higher gain on coefficients from a particular band, then changes in that band will disproportionately affect \( z \).

\section{Concluding Remarks and Further Directions}

To summarize, even if an explicit analysis in the literature might be scarce, a theoretical approach can be outlined as follows:
\begin{enumerate}
    \item \textbf{Linearize the diffusion mapping:} Use the Jacobian \( J_E(x) \) to capture local sensitivity.
    \item \textbf{Decompose perturbations in the wavelet domain:} Exploit the linearity and orthogonality of the wavelet transform.
    \item \textbf{Analyze the composite mapping \( A = J_E(x)\, W^{-1} \):} This operator relates changes in wavelet coefficients (across frequency bands) to changes in the diffusion latent space.
\end{enumerate}

Future work might involve numerically computing the Jacobian for trained diffusion models, decomposing it in the wavelet domain, and studying its spectral properties to understand how different frequency bands contribute to the latent representation. This analysis could shed light on phenomena such as the ``spectral bias'' of generative models or the robustness of reconstructions across scales.

This theoretical framework provides a starting point for a deeper investigation into how the interplay between wavelet frequency bands and the diffusion process affects the latent representations.


==> Sec/theory_1.tex <==
\section{Theoretical jutification}

\begin{lemma}[Orthogonality of Subbands]
Let \( x \in \mathbb{R}^n \) be a latent representation decomposed into \( k \) orthogonal subbands \( \{P_l(x)\}_{l=1}^k \) using a frequency transform \( F \). Then, for any two distinct subbands \( l \neq l' \), we have:
\[
\langle P_l(x), P_{l'}(x) \rangle = 0.
\]
This orthogonality ensures that the contributions of each subband are independent, preventing cross-interference in the latent space.
\end{lemma}

\begin{theorem}[Reduction of concept interference in composite images]
Let \( x = \sum_{l=1}^k P_l(x) \) be a latent representation decomposed into \( k \) orthogonal subbands, where each subband encodes distinct concepts. Let \( S_{l}(x) \) denote the score function in the frequency domain for concept \( l \). When combining \( k \) distinct concepts into a single composite image, the guided update in the frequency domain reduces concept interference as:
\[
S_{l}(x) = S_{l, \text{uncond}}(x) + \alpha_l \big(S_{l, \text{cond}}(x) - S_{l, \text{uncond}}(x)\big)
\]

such that for any two distinct subbands \( l \neq l' \), the interference term is minimized as:
\[
\langle S_{l}(x), S_{l'}(x) \rangle = 0.
\]
\end{theorem}

% \begin{proof} 
% By Lemma 1, the subbands are orthogonal:
% \[
% \langle P_l(x), P_{l'}(x) \rangle = 0, \quad \forall l \neq l'.
% \]

% In naive CFG, the guidance update is applied globally:
% \[
% S(x) = S_{\text{uncond}}(x) + \gamma \big(S_{\text{cond}}(x) - S_{\text{uncond}}(x)\big)
% \]
% The global scaling \( \gamma \) applies uniformly across all components, causing interference as each concept influences the entire latent space.
 
% In frequency guidance, the update for each subband is:
% \[
% S_{l}(x) = S_{l, \text{uncond}}(x) + \alpha_l \big(S_{l, \text{cond}}(x) - S_{l, \text{uncond}}(x)\big)
% \]
% Since each \( S_{l}(x) \) is restricted to its respective subband, the cross-subband interaction term \( \langle S_{l}(x), S_{l'}(x) \rangle \) remains zero due to orthogonality.

% For naive CFG, the variance of the combined signal is given by:
% \[
% \text{Var}(S(x)) = \sum_{l=1}^k \text{Var}(S_{l}(x)) + \sum_{l \neq l'} \text{Cov}(S_{l}(x), S_{l'}(x))
% \]
% In frequency guidance, due to orthogonality, the covariance terms vanish:
% \[
% \text{Var}(S(x)) = \sum_{l=1}^k \text{Var}(S_{l}(x))
% \]
% Thus, the influence of each concept is confined to its specific subband, preventing destructive interference and ensuring clearer separation of visual attributes.
% \end{proof}

\textit{Proof.} The proof is provided in the Appendix. The interpretation of this result is when combining multiple concepts into a single composite image, frequency guidance leverages orthogonal subbands to isolate each concept’s contribution, minimizing cross-concept interference. This structured decomposition ensures that each concept is treated independently, effectively reducing interference compared to the naive CFG approach where all concepts interact globally in the latent space.

==> Sec/theory_2.tex <==
\section{Theoretical jutification}
\begin{lemma}[Weighted Orthogonality of Subbands]
Let \( x \in \mathbb{R}^n \) be a latent representation decomposed into \( k \) subbands \( \{P_l(x)\}_{l=1}^k \) using a frequency transform \( F \). For each subband \( l \), we define a relevance score \( w_l \in [0, 1] \), indicating the proportion of the concept that resides within that subband. The weighted orthogonality condition is defined as:
\[
\langle P_l(x), P_{l'}(x) \rangle = w_l \cdot w_{l'} \cdot \text{Cov}(P_l(x), P_{l'}(x))
\]
where \( \text{Cov}(P_l(x), P_{l'}(x)) \) is the covariance between subbands \( l \) and \( l' \). If \( w_l \approx 0 \) for subband \( l \), its contribution to interference is minimal.
\end{lemma}

\begin{theorem}[Minimization of Concept Interference in Composite Images]
Let \( x = \sum_{l=1}^k P_l(x) \) be a latent representation decomposed into \( k \) subbands, where each subband may encode multiple concepts. Let \( S_{l}(x) \) denote the score function in the frequency domain for concept \( l \). When combining \( k \) distinct concepts, the interference between subbands is minimized by weighting each subband based on its relevance to the target concept:
\[
S_{l}(x) = S_{l, \text{uncond}}(x) + \alpha_l \cdot w_l \big(S_{l, \text{cond}}(x) - S_{l, \text{uncond}}(x)\big)
\]
where \( \alpha_l \) is the guidance scale for subband \( l \), and \( w_l \in [0, 1] \) is the relevance weight. Thus, the cross-subband interaction is minimized as:
\[
\langle S_{l}(x), S_{l'}(x) \rangle = w_l \cdot w_{l'} \cdot \text{Cov}(S_{l}(x), S_{l'}(x))
\]
\end{theorem}

% \begin{proof}
% 1. \textbf{Weighted Orthogonality Analysis:} From Lemma 1, the weighted orthogonality is expressed as:
% \[
% \langle P_l(x), P_{l'}(x) \rangle = w_l \cdot w_{l'} \cdot \text{Cov}(P_l(x), P_{l'}(x))
% \]
% If \( w_l \approx 0 \), the covariance term contributes minimally to cross-subband interference.

% 2. \textbf{Frequency Guidance Update:} The guidance update for each subband is defined as:
% \[
% S_{l}(x) = S_{l, \text{uncond}}(x) + \alpha_l \cdot w_l \big(S_{l, \text{cond}}(x) - S_{l, \text{uncond}}(x)\big)
% \]
% Each subband update is scaled by the relevance weight \( w_l \), controlling its impact on the overall composition.

% 3. \textbf{Variance Analysis:}
% For naive CFG, the variance of the combined signal is given by:
% \[
% \text{Var}(S(x)) = \sum_{l=1}^k \text{Var}(S_{l}(x)) + \sum_{l \neq l'} \text{Cov}(S_{l}(x), S_{l'}(x))
% \]
% In the frequency-guided setting with weighted orthogonality, the covariance term becomes:
% \[
% \text{Cov}(S_{l}(x), S_{l'}(x)) = w_l \cdot w_{l'} \cdot \text{Cov}(S_{l}(x), S_{l'}(x))
% \]
% Thus, by minimizing the weights \( w_l \) for subbands not relevant to the target concept, interference is effectively controlled.
% \end{proof}

\textit{Proof.} The proof is provided in the Appendix. The theoretical result establishes that by assigning relevance weights to subbands based on concept distribution, we effectively reduce cross-subband interference. Instead of assuming strict orthogonality, we leverage weighted covariance to minimize interactions in less relevant subbands, thereby enhancing the compositional fidelity of the combined image.


==> Sec/theory_3.tex <==
\section{Theoretical Analysis}

\begin{lemma}[Frequency Decomposition Reduces Interference]
Let \( x \) represent an image composed of multiple concepts \( \{c_i\}_{i=1}^n \). Consider wavelet decomposition of the image into frequency-specific subbands \( b \in \{LL, LH, HL, HH\} \):
\[
x = \sum_{b \in \{LL,LH,HL,HH\}} x_b.
\]
Define interference between concepts \( c_i \) and \( c_j \) within a subband \( b \) as:
\[
I_b(c_i, c_j) = \frac{\langle x_b^{c_i}, x_b^{c_j} \rangle}{\|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2}.
\]
Then, interference in the frequency domain is strictly lower than the spatial domain interference:
\[
|I_b(c_i, c_j)| \leq |I_{\text{spatial}}(c_i, c_j)|,
\]
with equality only if \( x_b^{c_i} \) and \( x_b^{c_j} \) perfectly align spatially and frequency-wise.
\end{lemma}

\begin{proof}
Wavelet decomposition inherently separates image features into distinct frequency subbands, capturing specific scales and textures independently. Consequently, this decomposition reduces the spatial overlap among features associated with different concepts. The cross-correlation within a single subband thus becomes significantly less than the cross-correlation computed directly in the spatial domain, ensuring reduced interference in the frequency representation.
\end{proof}

\begin{theorem}[Wavelet Frequency Decomposition-based Composition Reduces Concept Interference During Reverse Denoising]
Consider a reverse denoising process, where at each timestep \( t \), an intermediate state \( x^t \) is generated. Let \( x_b^t \) denote its wavelet frequency-specific subbands, and define adaptive composition weights as:
\[
w_b^{c_i,t} = \frac{\|\Delta x_b^{c_i,t}\|_2^2}{\sum_{j}\|\Delta x_b^{c_j,t}\|_2^2},
\]
where \(\Delta x_b^{c_i,t}\) represents the change in the frequency-specific subband for concept \( c_i \) at timestep \( t \). The frequency-domain guided composition is defined as:
\[
x_b^t = \sum_i w_b^{c_i,t} x_b^{c_i,t}.
\]
Then, the wavelet frequency decomposition combined with adaptive weights systematically reduces concept interference during the reverse denoising process.
\end{theorem}

\begin{proof}
By Lemma 1, wavelet decomposition already reduces interference by isolating concept features in frequency subbands. The adaptive weighting further minimizes interference by dynamically prioritizing frequency components that exhibit significant temporal changes, which reflect emerging or salient concept details during denoising. This temporal-frequency adaptive guidance ensures that dominant concept features are coherently emphasized at relevant denoising stages, systematically minimizing interference and improving the overall compositional integrity throughout the denoising process.
\end{proof}

==> Sec/theory_4.tex <==
\section{Theoretical Analysis}

\begin{lemma}[Frequency Decomposition Reduces Interference]
Let \( x \) represent an image composed of multiple concepts \( \{c_i\}_{i=1}^n \). Consider wavelet decomposition of the image into frequency-specific subbands \( b \in \{LL, LH, HL, HH\} \):
\[
x = \sum_{b \in \{LL,LH,HL,HH\}} x_b.
\]
Define interference between concepts \( c_i \) and \( c_j \) within a subband \( b \) as:
\[
I_b(c_i, c_j) = \frac{\langle x_b^{c_i}, x_b^{c_j} \rangle}{\|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2}.
\]
Then, interference in the frequency domain is strictly lower than the spatial domain interference:
\[
|I_b(c_i, c_j)| \leq |I_{\text{spatial}}(c_i, c_j)|,
\]
with equality only if \( x_b^{c_i} \) and \( x_b^{c_j} \) perfectly align spatially and frequency-wise.
\end{lemma}

\begin{proof}
Consider the spatial domain representations \( x^{c_i} \) and \( x^{c_j} \) for two distinct concepts \( c_i \) and \( c_j \). By the Cauchy–Schwarz inequality:
\[
|\langle x^{c_i}, x^{c_j} \rangle| \leq \|x^{c_i}\|_2 \|x^{c_j}\|_2.
\]
Equality holds only when \( x^{c_i} \) and \( x^{c_j} \) are linearly dependent. After wavelet decomposition, the spatial domain vectors are partitioned into frequency-specific vectors \( x_b^{c_i} \) and \( x_b^{c_j} \). Thus:
\[
|\langle x_b^{c_i}, x_b^{c_j} \rangle| \leq \|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2.
\]
Because wavelet decomposition distributes the original spatial features into separate subbands, reducing direct spatial overlap, it follows that:
\[
|I_b(c_i, c_j)| = \frac{|\langle x_b^{c_i}, x_b^{c_j} \rangle|}{\|x_b^{c_i}\|_2 \|x_b^{c_j}\|_2} \leq \frac{|\langle x^{c_i}, x^{c_j} \rangle|}{\|x^{c_i}\|_2 \|x^{c_j}\|_2} = |I_{\text{spatial}}(c_i, c_j)|.
\]
Equality is only achieved when \( x_b^{c_i} \) and \( x_b^{c_j} \) precisely align in both frequency and spatial domains, which is highly unlikely in practice due to the nature of wavelet decomposition.
\end{proof}

\begin{theorem}[Wavelet Frequency Decomposition-based Composition Reduces Concept Interference During Reverse Denoising]
Consider a reverse denoising process, where at each timestep \( t \), an intermediate state \( x^t \) is generated. Let \( x_b^t \) denote its wavelet frequency-specific subbands, and define adaptive composition weights as:
\[
w_b^{c_i,t} = \frac{\|\Delta x_b^{c_i,t}\|_2^2}{\sum_{j}\|\Delta x_b^{c_j,t}\|_2^2},
\]
where \(\Delta x_b^{c_i,t}\) represents the change in the frequency-specific subband for concept \( c_i \) at timestep \( t \). The frequency-domain guided composition is defined as:
\[
x_b^t = \sum_i w_b^{c_i,t} x_b^{c_i,t}.
\]
Then, the wavelet frequency decomposition combined with adaptive weights systematically reduces concept interference during the reverse denoising process.
\end{theorem}

\begin{proof}
By Lemma 1, wavelet decomposition already reduces interference by isolating concept features in frequency subbands. The adaptive weighting further minimizes interference by dynamically prioritizing frequency components that exhibit significant temporal changes, which reflect emerging or salient concept details during denoising. This temporal-frequency adaptive guidance ensures that dominant concept features are coherently emphasized at relevant denoising stages, systematically minimizing interference and improving the overall compositional integrity throughout the denoising process.
\end{proof}


==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


